STX-Vote: Improving Reliability with Bit Voting in Synchronous Transmission-based IoT Networks

Industrial Internet of Things (IIoT) networks must meet strict reliability, latency, and low energy consumption requirements. However, traditional low-power wireless protocols are ineffective in finding a sweet spot for balancing these performance metrics. Recently, network flooding protocols based on Synchronous Transmissions (STX) have been proposed for better performance in reliability-critical IIoT, where simultaneous transmissions are possible without packet collisions. STX-based protocols can offer a competitive edge over routing-based protocols, particularly in dependability. However, they notably suffer from the beating effect, a physical layer phenomenon that results in sinusoidal interference across a packet and, consequently, packet loss. Thus, we introduce STX-Vote, an error correction scheme that can handle errors caused by beating effects. Importantly, we utilize transmission redundancy already inherent within STX protocols so do not incur additional on-air overhead. Through simulation, we demonstrate STX-Vote can provide a 40% increase in reliability. We subsequently implement STX-Vote on nRF52840-DK devices and perform extensive experiments. The results confirm that STX-Vote improves reliability by 25-28% for BLE 5 PHYs and 8% for IEEE 802.15.4; thus, it can complement existing error correction schemes.

==> Images.tex <==
contains the images that were removed from the paper.


% \begin{figure*}[ht]
%     \centering
%     % \hspace{-50pt}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/1M/PHY_BLE_1M_error_positions_20240109_1253.pdf}
%         \caption{Pair-1 1M}
%         \label{fig:beating_1m_pic1}
%     \end{subfigure}
%     \begin{subfigure} [ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/1M/PHY_BLE_1M_error_positions_20240109_1257.pdf}
%         \caption{Pair-2 1M}
%         \label{fig:beating_1m_pic2}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/1M/PHY_BLE_1M_error_positions_20240109_1303.pdf}
%         \caption{Pair-3 1M}
%         \label{fig:beating_1m_pic3}
%     \end{subfigure}
%     \begin{subfigure} [ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/1M/PHY_BLE_1M_error_positions_20240109_1307.pdf}
%         \caption{Pair-4 1M}
%         \label{fig:beating_1m_pic4}
%     \end{subfigure}

%     \begin{subfigure}[ht]{0.12\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/2M/PHY_BLE_2M_error_positions_20240109_1253.pdf}
%         \caption{Pair-1 2M}
%         \label{fig:beating_n16_2m_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/2M/PHY_BLE_2M_error_positions_20240109_1258.pdf}
%         \caption{Pair-2 2M}
%         \label{fig:beating_n16_2m_pic2}
%     \end{subfigure}
%     \begin{subfigure} [ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/2M/PHY_BLE_2M_error_positions_20240109_1304.pdf}
%         \caption{Pair-3 2M}
%         \label{fig:beating_n16_2m_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/2M/PHY_BLE_2M_error_positions_20240109_1308.pdf}
%         \caption{Pair-4 2M}
%         \label{fig:beating_n16_2m_pic4}
%     \end{subfigure}
    
%     \begin{subfigure}[ht]{0.12\textwidth}
%          \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/125K/PHY_BLE_125K_error_positions_20240109_1252.pdf}
%         \caption{Pair-1 125K}
%         \label{fig:beating_n16_125K_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/125K/PHY_BLE_125K_error_positions_20240109_1259.pdf}
%         \caption{Pair-2 125K}
%         \label{fig:beating_n16_125K_pic2}
%     \end{subfigure}
%     \begin{subfigure} [ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/125K/PHY_BLE_125K_error_positions_20240109_1305.pdf}
%         \caption{Pair-3 125K}
%         \label{fig:beating_n16_125K_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/125K/PHY_BLE_125K_error_positions_20240109_1309.pdf}
%         \caption{Pair-4 125K}
%         \label{fig:beating_n16_125K_pic4}
%     \end{subfigure}
    
%     \begin{subfigure}[ht]{0.12\textwidth}
%          \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/500K/PHY_BLE_500K_error_positions_20240109_1254.pdf}
%         \caption{Pair-1 500K}
%         \label{fig:beating_n16_500k_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/500K/PHY_BLE_500K_error_positions_20240109_1300.pdf}
%         \caption{Pair-2 500K}
%         \label{fig:beating_n16_500k_pic2}
%     \end{subfigure}
%     \begin{subfigure} [ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/500K/PHY_BLE_500K_error_positions_20240109_1306.pdf}
%         \caption{Pair-3 500K}
%         \label{fig:beating_n16_500k_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/500K/PHY_BLE_500K_error_positions_20240109_1309.pdf}
%         \caption{Pair-4 500K}
%         \label{fig:beating_n16_500k_pic4}
%     \end{subfigure}
    
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/IEEE/PHY_IEEE_error_positions_20240109_1256.pdf}
%         \caption{Pair-1 IEEE}
%         \label{fig:beating_n16_ieee_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/IEEE/PHY_IEEE_error_positions_20240109_1300.pdf}
%         \caption{Pair-2 IEEE}
%         \label{fig:beating_n16_ieee_pic2}
%     \end{subfigure}
%     \begin{subfigure} [ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/IEEE/PHY_IEEE_error_positions_20240109_1306.pdf}
%         \caption{Pair-3 IEEE}
%         \label{fig:beating_n16_ieee_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.12\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg16dBm/IEEE/PHY_IEEE_error_positions_20240109_1310.pdf}
%         \caption{Pair-4 IEEE}
%         \label{fig:beating_n16_ieee_pic4}
%     \end{subfigure}
%     \caption{A mixture of wide and narrow beating is seen for uncoded BLE physical layers due to different CFO between different CTX pairs. For coded BLE 5 physical layers and \ieee beating appears to be wide as there are no distinct crests or valleys seen in comparison to uncoded BLE5 physical layers.}
%     \label{beating_pic}
%     \vspace{-4mm}
% \end{figure*}



% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/125K/PHY_BLE_125K_error_positions_20240109_1313.pdf}
%         \caption{Pair-1 125K}
%         \label{fig:beating_n20_125K_pic1}
%         \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/125K/PHY_BLE_125K_error_positions_20240109_1316.pdf}
%         \caption{Pair-2 125K}
%         \label{fig:beating_n20_125K_pic2}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/125K/PHY_BLE_125K_error_positions_20240109_1320.pdf}
%         \caption{Pair-3 125K}
%         \label{fig:beating_n20_125K_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/125K/PHY_BLE_125K_error_positions_20240109_1323.pdf}
%         \caption{Pair-4 125K}
%         \label{fig:beating_n20_125K_pic4}
%     \end{subfigure}
    
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/500K/PHY_BLE_500K_error_positions_20240109_1314.pdf}
%         \caption{Pair-1 500K}
%         \label{fig:beating_n20_500K_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/500K/PHY_BLE_500K_error_positions_20240109_1317.pdf}
%         \caption{Pair-2 500K}
%         \label{fig:beating_n20_500K_pic2}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/500K/PHY_BLE_500K_error_positions_20240109_1321.pdf}
%         \caption{Pair-3 500K}
%         \label{fig:beating_n20_500K_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/500K/PHY_BLE_500K_error_positions_20240109_1324.pdf}
%         \caption{Pair-4 500K}
%         \label{fig:beating_n20_500K_pic4}
%     \end{subfigure}
    
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/IEEE/PHY_IEEE_error_positions_20240109_1314.pdf}
%         \caption{Pair-1 IEEE}
%         \label{fig:beating_n20_ieee_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/IEEE/PHY_IEEE_error_positions_20240109_1318.pdf}
%         \caption{Pair-2 IEEE}
%         \label{fig:beating_n20_ieee_pic2}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/IEEE/PHY_IEEE_error_positions_20240109_1321.pdf}
%         \caption{Pair-3 IEEE}
%         \label{fig:beating_n20_ieee_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/IEEE/PHY_IEEE_error_positions_20240109_1325.pdf}
%         \caption{Pair-4 IEEE}
%         \label{fig:beating_n20_ieee_pic4}
%     \end{subfigure}
%     \caption{The beating patterns using all coded BLE physical-layers and IEEE802.15.4. at -20dBm transmission power. Here we cannot see a distinct envelope for BLE5 125K and BLE5 500K because the transmission is lying in a beating valley indicating wide beating between the transmitting devices.}
%     \label{beating_pic_2_n20}
% \end{figure*}


% \begin{figure*} [ht]
%     \centering
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/1M/PHY_BLE_1M_error_positions_20240109_1312.pdf}
%         \caption{Pair-1 1M}
%         \label{fig:beating_n20_1m_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/1M/PHY_BLE_1M_error_positions_20240109_1319.pdf}
%         \caption{Pair-2 1M}
%         \label{fig:beating_n20_1m_pic2}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/1M/PHY_BLE_1M_error_positions_20240109_1322.pdf}
%         \caption{Pair-3 1M}
%         \label{fig:beating_n20_1m_pic3}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/2M/PHY_BLE_2M_error_positions_20240109_1312.pdf}
%         \caption{Pair-1 2M}
%         \label{fig:beating_n20_2m_pic1}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/2M/PHY_BLE_2M_error_positions_20240109_1319.pdf}
%         \caption{Pair-2 2M}
%         \label{fig:beating_n20_2m_pic2}
%     \end{subfigure}
%     \begin{subfigure}[ht]{0.16\textwidth}
%         \includegraphics[width=\columnwidth]{figures/Neg20dBm/2M/PHY_BLE_2M_error_positions_20240109_1323.pdf}
%         \caption{Pair-3 2M}
%         \label{fig:beating_n20_2m_pic3}
%     \end{subfigure}
%     \caption{The beating patterns in all uncoded BLE physical-layers.In this setting we did not see beating for one of the selected pairs in uncoded BLE physical-layers as they were not able to sync because of high packet distortion due to beating and low transmission power.}
%     \label{beating_pic_1_n20}
%     % \vspace{-8mm}
% \end{figure*}
